A Unique Messenger to Probe Active Galactic Nuclei: High-Energy Neutrinos

This Astro2020 white paper advocates for a multi-messenger approach that combines high-energy neutrino and broad multi-wavelength electromagnetic observations to study AGN during the coming decade. The unique capabilities of these joint observations promise to solve several long-standing issues in our understanding of AGN as powerful cosmic accelerators.

==> cover.tex <==
\raggedright

\Large
Astro2020 Science White Paper \linebreak

\textbf{Probing High-Energy Neutrino Emission from Active Galactic Nuclei in the Coming Decade} \linebreak
\normalsize

\noindent \textbf{Thematic Areas:} Multi-Messenger Astronomy and Astrophysics
\linebreak
  
\textbf{Authors:} Marcos Santander, Thomas Maccarone, Nathan Whitehorn, Azadeh Keivani \\
Kohta Murase, Maria Petropoulou,  Ignacio Taboada, Lorenzo Sironi, Ke Fang \\
Sara Buson, Derek Fox, your name here...

Name:	
 \linebreak						
Institution:  
 \linebreak
Email: 
 \linebreak
Phone:  
 \linebreak
 
\textbf{Endorsers:} 
  \linebreak



%\begin{figure}[h]
%\centering
%\includegraphics[width=0.65\textwidth]{BlazarNeutrino2_1920x1080_M.jpg}
%\caption{NuBlazar}
%\label{NuBlazar}
%\end{figure}

\justify
\textbf{Abstract:} Recent multi-messenger studies involving electromagnetic and neutrino observations have provided compelling evidence for blazars, a subclass of active galactic nuclei (AGN), as high-energy neutrino emitters. These observations could have significant ramifications for high-energy astrophysics, as they would signify the dawn of high-energy neutrino astronomy, resolve the long-standing question of the origin of cosmic rays, and help ellucidate the processes responsible for the emission observed from blazars and other active galactic nuclei. The continued operation of existing electromagnetic and neutrino observatories, as well as the start of operation of several new ones in currently-unexplored energy bands, promises to solve several of these questions over the coming decade. This white paper outlines the scientific case for multi-messenger studies of blazars and other AGN using EM and neutrino observations and provides an outlook of what new observations will tell us about these extreme objects. 

\pagebreak
